Combinatoire alg\'ebrique li\'ee aux ordres sur les permutations

This thesis comes within the scope of algebraic combinatorics and studies problems related to three orders on permutations: the two said weak orders (right and left) and the strong order or Bruhat order. The first part deals with bases of multivariate polynomials. Most specifically, we study a product of Grothendieck polynomials and prove that it can interpreted as a sum over the Bruhat order. We also present our implementation of Grothendieck polynomials and other bases in Sage. In a second part, we study the Tamari order binary trees. We obtain a new enumeration formula on the Tamari lattice and a new combinatorial prove of Chapoton's functional equation of the generating functions of Tamari intervals. We extend our results to the m-Tamari case and thus retrieve a formula given by Bousquet-M\'elou, Pr\'eville-Ratelle and Fusy.

==> includes/figures/interval-posets/I3-ex3.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\def \hlev {1}
\def \wlev {1}

\begin{tikzpicture}
	\node(T11) at (0,-1 * \hlev){1};
      \node(T12) at (0.5 * \wlev,0){2};
      \node(T13) at (\wlev,-1 * \hlev){3};
      \draw(T13) -- (T12);
      \draw(T11) -- (T12);
\end{tikzpicture}

==> includes/figures/interval-posets/I4-ex1.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\begin{tikzpicture}
\node(T21) at (0,0){1};
      \node(T23) at (1,0){3};
      \node(T22) at (0.5,-1){2};
      \node(T24) at (1.5,-1) {4};
      \draw(T22) -- (T23);
      \draw(T24) -- (T23);
\end{tikzpicture}

==> includes/figures/mbinary/P2-2-a-inv-n.tex <==
% Auteur : Viviane Pons
% Création 21/05/2013

%        .
%      ./ \.
%        ./

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){1};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (3.500, -1.000){2};
\node (N010) at (2.500, -2.000){2};
\draw (N01) -- (N010);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/mbinary/P2-2-b-inv-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./\.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){2};
\node (N00) at (1.500, -1.000){1};
\node (N000) at (0.500, -2.000){1};
\node (N001) at (2.500, -2.000){2};
\draw (N00) -- (N000);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/mbinary/P2-2-c-inv-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%      /
%     /
%    /

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){2};
\node (N00) at (2.500, -1.000){2};
\node (N000) at (1.500, -2.000){1};
\node (N0000) at (0.500, -3.000){1};
\draw (N000) -- (N0000);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T2-1.tex <==
% Auteur : Viviane Pons
% Création : 11/05/2013

%     .
%   ./

\begin{tikzpicture}
\node (N0) at (0.750, 0.000){};
\node (N00) at (0.250, -0.500){};
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> includes/figures/trees/T3-1-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T3-1.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (1.250, 0.000){};
\node (N00) at (0.750, -0.500){};
\node (N000) at (0.250, -1.000){};
\draw[Point] (N000) circle;
\draw (N00.center) -- (N000.center);
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> includes/figures/trees/T3-2-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%      \.

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T3-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T3-4-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%     ./ \.
%       

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T3-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-1-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%      /
%     /
%    /

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (1.500, -2.000){2};
\node (N0000) at (0.500, -3.000){1};
\draw (N000) -- (N0000);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-10-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%      ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\node (N0100) at (1.500, -3.000){2};
\draw (N010) -- (N0100);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-11-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%         \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (1.500, -2.000){2};
\node (N0101) at (2.500, -3.000){3};
\draw (N010) -- (N0101);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-12-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%         \.
%        ./ \.
%        

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\node (N011) at (3.500, -2.000){4};
\draw (N01) -- (N010);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-13-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%           \.
%          ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (3.500, -2.000){4};
\node (N0110) at (2.500, -3.000){3};
\draw (N011) -- (N0110);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-14-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%         \.
%           \.
%             \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\node (N0111) at (3.500, -3.000){4};
\draw (N011) -- (N0111);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-2-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./
%     \

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (0.500, -2.000){1};
\node (N0001) at (1.500, -3.000){2};
\draw (N000) -- (N0001);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./\.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\node (N001) at (2.500, -2.000){3};
\draw (N00) -- (N000);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-4-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%       \.
%      ./

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (2.500, -2.000){3};
\node (N0010) at (1.500, -3.000){2};
\draw (N001) -- (N0010);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%      ./
%       \.
%        \.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\node (N0011) at (2.500, -3.000){3};
\draw (N001) -- (N0011);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-6-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%     ./

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\node (N01) at (3.500, -1.000){4};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-7-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%       \.

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\node (N01) at (3.500, -1.000){4};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-8-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%        ./

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\draw (N01) -- (N010);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-9-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%           \.

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N011) at (3.500, -2.000){4};
\draw (N01) -- (N011);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}
